Development and Application of QM/MM Methods with Advanced Polarizable Potentials

Quantum Mechanics/Molecular Mechanics (QM/MM) simulations are a popular approach to study various features of large systems. A common application of QM/MM calculations is in the investigation of reaction mechanisms in condensed-phase and biological systems. The combination of QM and MM methods to represent a system gives rise to several challenges that need to be addressed. The increase in computational speed has allowed the expanded use of more complicated and accurate methods for both QM and MM simulations. Here, we review some approaches that address several common challenges encountered in QM/MM simulations with advanced polarizable potentials, from methods to account for boundary across covalent bonds and long-range effects, to polarization and advanced embedding potentials.

==> Figures/figure-aniline-path.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[H]

%\captionsetup{justification=raggedright,singlelinecheck=false}
%\captionsetup{justification=justified}
%\begin{center}


%\includegraphics[width=\textwidth]{Figures/aniline-reaction.png}


%\caption{Reaction scheme for the N-tert-butoxycarbonylation of aniline. Panel (1) describes the step–wise mechanism and panel (2) describes the concerted mechanism mentioned above. Reproduced from Vazquez-Montelongo, E.A.; Vazquez-Cervantes, J.E.; Cisneros, G.A. Current Status of AMOEBA–IL: A Multipolar/Polarizable Force Field for Ionic Liquids. Int. J. Mol. Sci. 2020, 21, 697. \cite{Vazquez-Montelongo2020}} 
%\label{fig:aniline-reaction}
%\end{center}
%\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[H]

\captionsetup{justification=raggedright,singlelinecheck=false}
%\captionsetup{justification=justified}
\begin{center}


\subfloat[]{\includegraphics[width=\textwidth]{Figures/aniline-reaction-scheme-c.png}
\label{fig:aniline-reaction-c}}


\subfloat[]{\includegraphics[width=.5\textwidth]{Figures/aniline-C2-scheme1c.jpg}
\label{aniline-1c-pol}}
\subfloat[]{\includegraphics[width=.5\textwidth]{Figures/figure-aniline-path-scheme-c.png}
\label{aniline-1c-no-pol}}


\subfloat[]{\includegraphics[width=\textwidth]{Figures/aniline-reaction-scheme-d.png}
\label{fig:aniline-reaction-d}}


\subfloat[]{\includegraphics[width=.5\textwidth]{Figures/aniline-C2-scheme1d.jpg}
\label{aniline-1d-pol}}
\subfloat[]{\includegraphics[width=.5\textwidth]{Figures/figure-aniline-path-scheme-d.png}
\label{aniline-1d-no-pol}}

\caption{
\protect\subref{fig:aniline-reaction-c} Reaction scheme for the N-tert-butoxycarbonylation of aniline for the step–wise mechanism. 
\protect\subref{aniline-1c-pol} Minimum energy path for Configuration C2, Scheme 1c.
\protect\subref{aniline-1c-no-pol} Minimum energy path for Scheme c for Configuration C2 without the AMOEBA polarization term.
\protect\subref{fig:aniline-reaction-d} Reaction scheme for the N-tert-butoxycarbonylation of aniline for the concerted mechanism.
\protect\subref{aniline-1d-pol} Minimum energy path for Configuration C2, Scheme 1d. 
\protect\subref{aniline-1d-no-pol} Minimum energy path for Scheme d for Configuration C2 without the AMOEBA polarization term.
Adapted from Vazquez-Montelongo, E.A.; Vazquez-Cervantes, J.E.; Cisneros, G.A. Polarizable ab initio QM/MM Study of the Reaction Mechanism of N-tert-Butyloxycarbonylation of Aniline in [EMIm][BF4]. Molecules 2018, 23, 2830. \cite{Vazquez-Montelongo2018}} 
\label{fig:aniline-path}
\end{center}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

